Decentralized Stochastic Multi-Player Multi-Armed Walking Bandits

Multi-player multi-armed bandit is an increasingly relevant decision-making problem, motivated by applications to cognitive radio systems. Most research for this problem focuses exclusively on the settings that players have \textit{full access} to all arms and receive no reward when pulling the same arm. Hence all players solve the same bandit problem with the goal of maximizing their cumulative reward. However, these settings neglect several important factors in many real-world applications, where players have \textit{limited access} to \textit{a dynamic local subset of arms} (i.e., an arm could sometimes be ``walking'' and not accessible to the player). To this end, this paper proposes a \textit{multi-player multi-armed walking bandits} model, aiming to address aforementioned modeling issues. The goal now is to maximize the reward, however, players can only pull arms from the local subset and only collect a full reward if no other players pull the same arm. We adopt Upper Confidence Bound (UCB) to deal with the exploration-exploitation tradeoff and employ distributed optimization techniques to properly handle collisions. By carefully integrating these two techniques, we propose a decentralized algorithm with near-optimal guarantee on the regret, and can be easily implemented to obtain competitive empirical performance.

==> algorithm.tex <==
\section{Proposed Algorithms}

    

\begin{table}
\caption{Summary of Notations}
\begin{center}
\begin{tabular}{ | m{6em} | m{5cm} | } 
  \hline
  Notations & Definitions\\ 
  \hline
 $\cN; N$ &Set of agents; number of agents \\ 
 $\cK; K$ &Set of arms; number of arms\\
 $T$ & Time Horizon\\
 $\mu_i$& Mean reward of arm $i$\\
 $X_{i,k}(t)$& Reward of arm $k$ by agent $i$ at time $t$\\
 $\hat{\mu}_{i,k}(t)$& Empirical estimation of reward of arm $k$ at agent $i$ till $t$\\
 $\mathcal{S}_{i}(t)$& The set of available arms by agent $i$ at time $t$\\
 $\cN_i$& Set of neighbor agents of agent $i$\\
 $I_{i,k}(t); C_{i,k}(t)$& Number of pulls and number of collisions for arm $k$ at agent $i$ till $t$;\\
 $B_{i,k}(t)$& Upper confidence bound for arm $k$ at agent $i$ at time $t$ \\
 $g_{i,k}(t)$& Index for exploration and exploitation 
 \\
  \hline
\end{tabular}
\end{center}
\end{table}

In this section, we propose two UCB-based algorithms for the considered (MA)$^2$B problem under two different communication frameworks. There are two common challenges for the (MA)$^2$B problem under this two frameworks: (i) how to maximize the accumulated reward in the face of unknown mean rewards, and (ii) how to avoid collision among different agents. 

To address the first challenge, the key is to balance the tradeoff between exploration and exploitation. We leverage the basic idea of UCB to address this challenge as follows.  
Let $I_{i,k}(t)$ be the number of times agent $i$ pulls arm $k$ by time $t$ and $C_{i,k}(t)$ be the number of times a collision occurs at agent $i$ when pulling arm $k$ by time $t$. Let $X_{i,k}(t)$ be the random reward received by agent $i$ when pulling arm $k$ at time $t$. Then we can define 
\begin{align}
\label{eq:esti_reward}
    \hat{\mu}_{i,k}(t)=\frac{\sum\limits_{\tau=1}^t\mathds{1}_{\{a_i(\tau)=k, a_n(\tau)\neq k, \forall n\neq i\}}X_{i,k}(\tau)}{I_{i,k}(t)-C_{i,k}(t)} 
\end{align}
as the local estimation of $\mu_k$ at agent $i$ up to time $t$, which is updated by agent $i$ itself. 
To accommodate the uncertainty of the estimation, we adopt the UCB technique by adding a perturbed term to the estimated average reward in \eqref{eq:esti_reward} and define 
\begin{align}\label{eq:index}
    g_{i,k}(t)=\hat{\mu}_{i,k}(t)+B_{i,k}(t),
\end{align}
where $B_{i,k}(t)$ is a function over $I_{i,k}(t)$ and $C_{i,k}(t)$.
The terms $\hat{\mu}_{i,k}(t)$ and $B_{i,m}(t)$ correspond to exploitation (pulling the arms with highest reward based on current estimation) and exploration (obtaining arms might gave improved higher reward), respectively. The $g_{i,k}(t)$ in \eqref{eq:index} is regarded as an index for decision making at the $i$-th agent's perspective. 
\begin{remark}
Though a UCB-based algorithm we proposed for the considered (MA)$^2$B in this paper,  there exists a  major difference compared with previous UCB-based techniques for (MA)$^2$B problem in which agents pull arms with the largest indices as defined in \eqref{eq:index}\cite{AMTS11,WPAJR20,boursier2019sic}. As presented later, each agent in our framework do not necessarily select the arm with largest index at each round $t$. The decision is made by jointly considering the current indices and the information shared by the neighbor agents. 
\end{remark}

As for the second challenge about the (MA)$^2$B setting, information sharing is needed to guarantee the sublinear accumulated regret as aforementioned. We consider two different settings: (i) each agent $i, \forall i \in\mathcal{N}$ only shares with its neighbor agents $\{j|j\in\mathcal{N}_j\}$ the information about  current available arm set $\mathcal{S}_i(t)$;
(ii)In addition to sharing $\mathcal{S}_i(t)$ to its neighbors, each agent $i$ also shares the estimated rewards of each arm to its neighbor agents $\{j|j\in\mathcal{N}_j\}$.
The first setting corresponds to the communication-limited scenario and the second setting represents communication-sufficient scenario. 




\subsection{Communication-Limited Framework}
 


We first present the framework in which the agents only have limited communication with their neighbors. 
Here, limited communication means that the agents can only share the information of the  available arm set among with the neighbors at each every round $t$ when arms sets change. The algorithm is dubbed as (MA)$^2$B-UCB.

Define $\mathcal{H}_i$ as a permutation of set of neighbors of agent $i$  and $\cH_i(m)$ denotes the $m$-th neighbor of agent $i$. Without loss of generality, we assume $\cH_i(1)=i.$ 
At each round $t$, agent $\cH_i(m), \forall m\in \big[|\mathcal{H}_i|\big]$ select exactly one arm $a_{im}$ from its available set $\mathcal{S}_{\cH_i(m)}(t)$. Denote the set containing all possible combinations as $\mathcal{U}_i(t)$, which is defined as
\begin{align}\nonumber
    \mathcal{U}_i(t)\triangleq&\Bigg\{\ba_i\Bigg|\ba_i=\big[a_{i,1}, \ldots,a_{i,{|\mathcal{H}_i|}}\big],a_{i,m}\in\mathcal{S}_{\mathcal{H}_i(m)}(t),\\
   &\qquad\qquad  a_{i,m}\neq a_{i,n}, \forall m,n\in [|\mathcal{H}_i|]\Bigg\}.\label{eq:Uset}
\end{align}
Then, at each round $t\in\{1,2,\ldots,T\}$, each agent $i, \forall i\in\mathcal{N}$ performs the following procedures.
\begin{enumerate}
    \item[1)] Observes the available arms set $\mathcal{S}_i(t)$ and transmits $\cS_i(t)$ to its neighbors $j\in\mathcal{N}_i$;
   Receives $\mathcal{S}_j(t), \forall j\in\mathcal{N}_j$ from its neighbors;
    \item[2)] Based on the local indices $\bg_i(t):=\{g_{i,k}(t), \forall k\in\cK\}$, agent $i$ will form an optimal pulling strategy by selecting one arm from each available arm set $\mathcal{S}_j(t), \forall j\in\mathcal{N}_i$ by solving 
\begin{align}\label{eq:mathcing}
    \ba_i^*=\arg\max_{\ba_i\in\mathcal{U}_i(t)}\sum_{m=1}^{|\mathcal{H}_i|}g_{i,a_{i,m}}(t).
\end{align}
   \item [3)] Agent $i$ pulls the arm $a_i(t)$ indicated by $\ba_i^*(1)$. 
   \item[4)] Agent $i$ update the count of pulling $I_{i,k}(t+1)$ and collision $C_{i,k}(t)$ for arm $k$ as follows
   \begin{align}\nonumber
     I_{i,k}(t+1)&= I_{i,k}(t)+\mathds{1}_{\{a_{i}(t)=k\}};\\
     C_{i,k}(t+1)&=C_{i,k}(t)+\mathds{1}_{\{X_{i,k}(t)=0\}}.\label{eq:count_update}
   \end{align}
   Agent $i$ also updates $\hat{\mu}_{i,k}(t+1)$ according to \eqref{eq:esti_reward} and $g_{i,k}(t+1)$ according to \eqref{eq:index}.
\end{enumerate}

\begin{remark}
The major complexity of these procedures comes from solving the matching problem in \eqref{eq:mathcing}. Because the cardinality of the set $\cU_i(t)$ is the product of the cardinality of each set $\cS_{\cH_i(m)}(t), \forall m\in [|\cH_i|]$, i.e., $|\cU_i(t)|=\prod_{m=1}^{|\cH_i|}|\cS_{\cH_i(m)}(t)|$, which exponentially increases as the number of neighbor agents $|\cH_i|$ and the number of arms for each set $\cS_{\cH_i(m)}(t), \forall m\in [|\cH_i|]$. To reduce the complexity, we design an efficient matching algorithm in Algorithm \ref{alg:Mathcing} for \eqref{eq:mathcing}. It turns out that the complexity for searching $\bo_i$ is linearly with $|\cA_i|$ and the complexity for recovering $\cU_i(t)$ from $\bo_i$ is less than $factorial(|\cH_i|)$.
\end{remark}
\begin{algorithm}
 
	\caption{Optimal Matching for \eqref{eq:mathcing}} 
	\label{alg:Mathcing}
	\textbf{Input:}
	The feasible arm sets $\{\mathcal{S}_j(t), \forall j\in \mathcal{N}_i\}$ at current round $t$; 
	the statistics $\{g_{i,k}(t),\forall k\in\mathcal{M}\}$; a permutation $\cH_i$ with $\cH_i(1)=i$; \\
	\textbf{Initialization:} $\cO_i(t)=\phi, \cX_i^\ell=\phi, \forall \ell\in[|\cH_i|]$;
   
	\begin{algorithmic}[1]
	  
	  \STATE Find  $\cA_i=\bigcup_{m=1}^{|\cH_i|}\cS_{\cH_i(m)}(t) $ and sort $\cA_i$ in a decreasing order based on the statistic $\{g_{i,k}(t), \forall k\in \cA_i\}$, i.e., $g_{i,\cA_i(1)}(t)\geq g_{i,\cA_i(2)}(t)\geq\ldots\geq g_{i,\cA_i(|\cA_i|)}(t).$	\FOR{$\ell=1,2,...,|\cH_i|$}
		
	
		
        \STATE Put the agent IDs containing $\cA_i(1)$ in $\cX_i^\ell$.\\
        
        \IF{$|\bigcup_{l=1}^\ell \cX_i^l|\geq \ell$} 
        \STATE $\cO_i(t)=\cO_i(t)\cup\cA_i(1), \cA_i=\cA_i\setminus\cA_i(1)$ and go to step 2;
        \ELSE 
        \STATE $\cA_i=\cA_i\setminus\cA_i(1), \cX_i^\ell=\phi$ and go to step 3; 
        \ENDIF

		\ENDFOR
		\STATE Return $\cU_i(t)$ according to \eqref{eq:Uset} by letting $\cS_{\cH_i(m)}(t)=\cS_{\cH_i(m)}(t)\cap \cO_i(t)$.
		\STATE Randomly select a policy from $\cU_i(t)$ as $\ba_i^*$.
	\end{algorithmic}
\end{algorithm}

Instead of finding all the possible combinations in $\cU_i(t)$ as in \eqref{eq:Uset}, the proposed matching algorithm in Algorithm \ref{alg:Mathcing} aims to find the optimal arm set $\cO_i(t)$ at agent $i$'s perspective first, where optimal means that by selecting any arms outside of $\cO_i(t)$, agents from $\cN_i$ will achieve a lower expected sum rewards at current round $t$. Then, agent $i$ only considers the combinations $\ba_i\in\cU_i$  with elements choosing from $\cO_i(t)$. Thus, any $\ba_i\in\cU_i$ is optimal for \eqref{eq:mathcing}. The detailed procedures are described below.


\begin{enumerate}
    \item[1)]
Agent $i$ forms the union set $\cA_i$ of all available arm set $\cS_j(t), j\in\cN_i$ and sort the arms in $\cA_i$ according to local statistics $g_{i,k}, \forall k\in \cN$ as shown at line 1. 
\item[2)] At line 2-9, agent $i$ matches arms from high order to low order according the order in $\cA_i$ until finding $|\cH_i|$ best arms for all agents in the neighborhood set $\cN_i$ at current round $t$.  
\item[3)] To determine if arm $\cA_i(1)$ is the $\ell$-th desired arm in $\cO_i(t)$ or not, agent $i$ needs firstly to find the set $\cX_i^\ell$ which contains all the agents who can pull arm $\cA_i(1)$, as shown at line 3.
\item[4)] At line 4-8, if there are no less than $\ell$ agents associated with arms in $\cO_i(t)\cup\cA_i(1)$, i.e., $|\bigcup_{l=1}^\ell \cX_i^l|\geq \ell$, it means $\cA_i(1)$ is a desired arm in $\cO_i(t)$, and thus agent $i$ updates the follows $\cO_i(t)=\cO_i(t)\cup\cA_i(1), \cA_i=\cA_i\setminus\cA_i(1)$; On the contrary, if there are less than $\ell$ agents associated with arms in $\cO_i(t)\cup\cA_i(1)$, i.e., $|\bigcup_{l=1}^\ell \cX_i^l|\leq \ell$, it means $\cA_i(1)$ is not an choice of set $\cO_i(t)$, and thus agent $i$ updates  $\cO_i(t)=\cO_i(t)\cup\cA_i(1), \cA_i=\cA_i\setminus\cA_i(1)$.
\item[5)] At line 10-11, agent $i$ construct $\cU_i(t)$ according to \eqref{eq:Uset} by only selecting arms from $\cO_i(t)$ and thus any $\ba_i$ from $\cU_i(t)$ is optimal for \eqref{eq:mathcing}.
\end{enumerate}
 
% \begin{algorithm}
 
% 	\caption{(MA)$^2$B-UCB: A single agent's perspective} 
% 	\label{alg:procedure}
% 	\textbf{Initialize:}
% 	The feasible arm sets  $\{\mathcal{S}_i(1), \forall i\in \mathcal{N}\}$; 
% 	the sample mean available at agent $i$ $\{\hat{\mu}_{i,k}(1)=0, \forall k\in\mathcal{N}\}$, and the statistics $\{g_{i,k}(1)=\infty,\forall k\in\mathcal{N}\}$;
% 	the number of pulls $\{I_{i,k}(1)=0, \forall i, k\}$ and the number of collisions $\{C_{i,k}(1)=0, \forall i, k\}$.
% 	\begin{algorithmic}[1]
% 		\FOR{$t=1,1,...,T$}
		
	
		
%         \STATE Transmit  $\mathcal{S}_i(t)$ to its neighbors and receive the information $\mathcal{S}_j(t)$ from all the neighbor agents $j\in\mathcal{N}_i$.\\
        
%         \STATE  Solving \eqref{eq:mathcing} by using Algorithm \ref{alg:Mathcing} and selects the arm indicated by $\ba_i^*(1)$. \\
        
        
%         \STATE Updates $I_{i,k}(t)$ and $C_{i,k}(t)$ according to \eqref{eq:count_update}.
        
%         \STATE Updates $\hat{\mu}_{i,k}(t+1)$ according to \eqref{eq:esti_reward} and $g_{i,k}(t+1)$ according to \eqref{eq:index}.
        
% 		\ENDFOR
% 	\end{algorithmic}
% \end{algorithm}
Notice that when the optimal policies in $\cU_i(t)$ indicates more than two different arms that agent $i$ can there are more than one optimal policy.  





\subsection{Communication-sufficient Framework}

Next, we  consider the communication-sufficient framework where each agent can not only share the available arm set, but also the empirical estimation of reward of each arm with its neighbors. This gives rise to the widely-adopted consensus based distributed learning procedure. This algorithm is dubbed as C(MA)$^2$B-UCB.


 Define $\tilde{r}_{i,k}(t)$ as the  estimation for average reward of arm $k$ at agent $i$ till time $t$. 
Agent $i$ maintains a local estimate of the parameter vector $\tilde{r}_{i,k}(t), \forall k$ at iteration $t$ and broadcasts it to its neighbors. The local estimate is updated as follows:
\begin{align}
\label{eq:local-estimation-all}
\tilde{r}_{i,k}({t+1})\!=\!\!\sum_{j\in \mathcal{N}_j} \!\tilde{r}_{j,k}(t)P_{i,j}\!+\! \hat{\mu}_{i,k}(t+1)-\hat{\mu}_{i,k}(t),
\end{align}
where $\bP=(P_{i,j})$ is a $N\times N$ non-negative matrix and we call it the \textit{consensus matrix}.   In other words, in each iteration, agent $i\in\cN$ computes a weighted average (i.e., consensus component) of the estimates of its neighbors and itself, and then corrects it by taking into account a stochastic approximation $(\hat{\mu}_i(t+1)-\hat{\mu}_i(t))$ of its local function. The weights are defined as
\begin{align}
\begin{cases}
P_{i,i}= 1-\sum_{j\in\mathcal{N}_i} P_{i,j},\\
P_{i,j}=\frac{1}{\max\{|\mathcal{N}_i|, |\mathcal{N}_j|\}}, \quad\text{if $j\in\mathcal{N}_i$},\\
P_{i,j}=0,\quad \text{otherwise}.
\end{cases}
\end{align}
Given the Metropolis weights,  $P$ are doubly stochastic, i.e., $\sum_{j=1}^N P_{i,j}=\sum_{i=1}^N P_{i,j}=1, \forall i, j.$

Then we can modify the index defined in \eqref{eq:index} by replacing $\hat{\mu}_{i,k}(t)$ into $\tilde{r}_{i,k}(t)$, i.e.,
\begin{align}\label{eq:index_consensus}
    g_{i,k}(t)=\tilde{r}_{i,k}(t)+B_{i,k}(t).
\end{align}
Provided this newly modified index, at each round $t$, agent $i, \forall i\in\mathcal{N}$ performs exactly same procedures as 1) - 4). The only difference is that each agent also receives $\tilde{r}_{j,k}(t), \forall k$ from its neighbors $j\in\mathcal{N}_j$ and update $\tilde{r}_{i,k}(t)$ according to \eqref{eq:local-estimation-all}. Hence, we directly
summarize the entire process in the following Algorithm \ref{alg:procedure2}. {\color{blue} Plan to make this algorithm fit to both settings}

\begin{algorithm}
 
	\caption{(MA)$^2$B-UCB: A single agent's perspective} 
	\label{alg:procedure2}
	\textbf{Initialize:}
	The feasible arm sets for each agent $\{\mathcal{S}_i(1), \forall i\in \mathcal{N}\}$; 
	the sample mean available at agent $i$ $\{\hat{\mu}_{i,k}(1)=0, \forall k\in\mathcal{N}\}$, and the statistics $\{g_{i,k}(1)=0,\forall k\in\mathcal{N}\}$;
	the number of pulls $\{I_{i,k}(1)=0, \forall i, k\}$ and the number of collisions $\{C_{i,k}(1)=0, \forall i, k\}$.
	\begin{algorithmic}[1]
		\FOR{$t=1,1,...,T$}
		
	
		
        \STATE Transmit t $\mathcal{S}_i(t)$ to its neighbors and receive the information $\mathcal{S}_j(t)$ from all the neighbor agents $j\in\mathcal{N}_i$.\\
        
        \STATE Update $\tilde{r}_{i,k}, \forall k$ according to \eqref{eq:local-estimation-all}.\\
        \STATE  Solving \eqref{eq:mathcing} to get the optimal pulling strategy $c_i^*(t)$ and selects the arm indicated by $c_i^*(t)$. \\
        
        
        \STATE Updates $I_{i,k}(t)$ and $C_{i,k}(t)$ according to \eqref{eq:count_update}.
        
        \STATE Updates $\hat{\mu}_{i,k}(t+1)$ according to \eqref{eq:esti_reward} and $g_{i,k}^*(t+1)$ according to \eqref{eq:index_consensus}.
        
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\begin{remark}

Define $\tilde{\br}_k:=[\tilde{r}_{1,k},  \ldots, \tilde{r}_{N,k}]^T$ and  $\hat{\pmb{\mu}}_k:=[\hat{\mu}_{1,k},  \ldots, \hat{\mu}_{N,k}]^T$as the vector stack of $\tilde{r}_{i,k}$ and $\hat{\mu}_{i,k}$, respectively. Then, we can simplify  \eqref{eq:local-estimation-all} as follows
\begin{align}
    \tilde{\br}_k(t+1)=\bP\tilde{\br}_k(t)+(\hat{\pmb{\mu}}_k(t+1)-\hat{\pmb{\mu}}_k(t)).
    \label{eq:matrix_form}
\end{align}
It it known that $\bP$ is irreducible  stochastic matrix such that there exists a rank-one matrix $\bP_\infty$ for which $\lim_{t\rightarrow \infty}\bP^t=\bP_\infty.$
\end{remark}

==> analysis.tex <==
\section{Theoretical Analysis}


To derive our main results, we first define the following parameters.  
Define $V_{i,j}(t)$ as the number of times in $t$ rounds where agent $i$ is the only agent to pull arm $j$. Hence the regret in \eqref{eq:regret} simplifies as
\begin{align}\label{eq:regret_def}
    R(T)=\sum_{t=1}^{T}\sum_{n=1}^{N}\mu_{a^*_n(t)}- \sum_{j=1}^M\sum_{i=1}^N\mu_j\mathbb{E}[V_{i,j}(T)].
\end{align}

For convenience, let $I_j(t):=\sum_{i=1}^N I_{i,j}(t)$ and $V_j(t):=\sum_{i=1}^N V_{i,j}(t)$. Note that $\sum_{j=1}^M I_j(T)=TN$. 
Denote $\cM_b$ as the set containing the first $N$-best arms, i.e., $\cM_b:=\{\mu_1, \mu_2, \ldots, \mu_N\}.$ The remaining arms are in the set $\mathcal{M}\setminus \cM_b$.
Define  $C(T):=\sum_{j\in \cM_b}I_j(T)-V_{j}(T)$ is the number of collisions faced by the agents in the $N$-best arms in $T$ rounds. Then we have the upper bound of regret in  following proposition.
\begin{proposition}
\label{prop:ub}
The accumulated regret after $T$ rounds is upper-bounded by
\begin{align}\nonumber
  R(T)\leq\mu_1\left(\mathbb{E}[C(T)]+ \sum_{j\in \cM\setminus\cM_b}\mathbb{E}[I_{j}(T)]\right),
\end{align}
\end{proposition}



To get the regret bound in Proposition \ref{prop:ub}, the key is to bound the time spent on each arm and the times that collision occurred for the $N$-best arms.

\begin{theorem}
\label{thm:A1}
The regret for Algorithm \ref{alg:procedure} is upper-bounded by
\begin{align*}
    R(T)&\leq \mu_1N\Bigg(\sum_{j\in\cM\setminus\cM_b}\sum_{k\in[M]\setminus j} \frac{12\log T}{(\mu_k-\mu_j)^2}\\
    &+\sum_{k=1}^N\sum_{m=k+1}^M \frac{12\log T}{(\mu_k-\mu_m)^2}+\frac{\pi^2}{3}M(M+N)\Bigg),
\end{align*}
with $ B_{i,k}(t)=\sqrt{\frac{3\log t}{V_{i,k}(t)}}$.
\end{theorem}


\begin{proofsketch}
Under this communication-limited scheme,
we can regard each agent is solving a MAB problem and
the total regret is bounded by the regret of each agent times
the number of agents. For a single agent $i$, the key is to bound the two factors $C_{i}(T)$ and $I_{i,j}(T), \forall j\in N \text{-worst}$ defined in Proposition \ref{prop:ub}. 
Observing that $ I_{i,j}(T)\leq \sum_{k\in [M]\setminus j}\sum_{t=1}^T\mathds{1}[g_{i,k}(t)\leq g_{i,j}(t)].$ A standard analysis in \cite{auer2002finite} can be leveraged for bounding each $\sum_{t=1}^T\mathds{1}[g_{i,k}(t)\leq g_{i,j}(t)]$. Due to the index sharing strategy, the collision occurs only when the statistical estimation is not accurate. Thus, the number of collision for each agent can be transferred to count for the number of inaccurate statistics, i.e., $\sum_{t=1}^T\mathds{1}[g_{i,k}(t)\leq g_{i,j}(t)], \forall k\geq j.$
\end{proofsketch}
\begin{remark}
The regret bound consists of two similar parts: counts for pulls of arms in the $N$-worst set and counts for collisions of arms in the $N$-best set. Each part is of order $\log(T)$ and linearly increasing with the number of agents $N$ and number of arm $M$, which is of the same order comparing with the existing work in \cite{AMTS11, WPAJR20}. Notice that previous work assumes that each agent has full access of the arms, such that collision s can be avoid without any communication between agents. However, under our considered moving arms, the collision will occur infinite often when there is no communication among neighbor agents. Nevertheless, by sharing only the available arm set information, we can still achieve sublinear $\log T$ regret. The communication overhead will not exceed $N^2M$ bits per round.

\end{remark}



\subsection{Analysis for Algorithm 2}



\begin{theorem}\label{thm:A2}
The regret for Algorithm \ref{alg:procedure2} is upper-bounded by
\begin{align*}
    &R(T)\leq \mu_1\Bigg(\sum_{i=1}^N\sum_{j\in\cM\setminus\cM_b}\sum_{k\in\mathcal{M}\setminus j}  \frac{12\log T}{|\mathcal{N}_i|(\mu_k-\mu_j)^2}\\
    &+\sum_{i=1}^N\sum_{k=1}^N\sum_{m=k+1}^M \frac{12\log T}{|\mathcal{N}_i|(\mu_k-\mu_m)^2}+\frac{\pi^2}{3}M(M+N)\Bigg),
\end{align*}
with $ B_{i,k}(t)=\sqrt{\frac{3\log t}{|\mathcal{N}_i|V_{i,k}(t)}}$.
\end{theorem}

\begin{proofsketch}
The proof follows similar step as that in Theorem \ref{thm:A1}. For a single agent $i$, the key is to bound the two factors $C_{i}(T)$ and $I_{i,j}(T), \forall j\in N \text{-worst}$ defined in Proposition \ref{prop:ub}. To bound those items, this proof makes use of important properties of sub-Gaussian random variables. Since any random variable with bounded support is sub-Gaussian, the empirical estimation $\hat{\mu}_{i,k}(t)$is sub-Gaussian. Hence, the consensus update $\tilde{r}_{i,k}(t)$ in \eqref{eq:local-estimation-all} is a linear combination of a set of sub-Gaussian random variables $\hat{\mu}_{i,k}(t)$, which is also sub-Gaussian due to the additivity property.   For any sub-Gaussian variable $\hat{\mu}_{i,k}(t)$, the key factor is the variance proxy $\sigma_{i,k}(t)$. After bounding the variance proxy $\sigma_{i,k}(t)$, we reuse the proof in Theorem \ref{thm:A1} to bound $C_i(T)$ and $I_{i,j}(T)$. This yields the regret upper bound.  
\end{proofsketch}

\begin{remark}
Similar with Theorem \ref{thm:A1}, Theorem \ref{thm:A2} also achieves a sublinear regret with respect to time horizon $T$. However, we can observe that when each agent communicates with the neighbors in terms of empirical estimation of rewards, the $T$-round accumulative regret can be decreased off in a factor of $\mathcal{O}(|\mathcal{N}_i|)$ for each agent $i$, which means that communication can improve the performance of the algorithm. This result is similar with that in \cite{ZL21} and \cite{SRJ17} when agents communicate with neighbors in a undirected graph and directed graph, respectively. The communication overhead is about $\tilde{\mathcal{O}}(N^2MT)$ for the whole process.
\end{remark}
